Independent Natural Policy Gradient Methods for Potential Games: Finite-time Global Convergence with Entropy Regularization

A major challenge in multi-agent systems is that the system complexity grows dramatically with the number of agents as well as the size of their action spaces, which is typical in real world scenarios such as autonomous vehicles, robotic teams, network routing, etc. It is hence in imminent need to design decentralized or independent algorithms where the update of each agent is only based on their local observations without the need of introducing complex communication/coordination mechanisms. In this work, we study the finite-time convergence of independent entropy-regularized natural policy gradient (NPG) methods for potential games, where the difference in an agent's utility function due to unilateral deviation matches exactly that of a common potential function. The proposed entropy-regularized NPG method enables each agent to deploy symmetric, decentralized, and multiplicative updates according to its own payoff. We show that the proposed method converges to the quantal response equilibrium (QRE) -- the equilibrium to the entropy-regularized game -- at a sublinear rate, which is independent of the size of the action space and grows at most sublinearly with the number of agents. Appealingly, the convergence rate further becomes independent with the number of agents for the important special case of identical-interest games, leading to the first method that converges at a dimension-free rate. Our approach can be used as a smoothing technique to find an approximate Nash equilibrium (NE) of the unregularized problem without assuming that stationary policies are isolated.

==> markov.tex <==
\section{Markov Potential Games}

\subsection{Background and formulation}
\paragraph{Markov Decision Process} A multi-agent MDP (or stochastic game) is formulated as $\mathcal{M} = \{\mathcal{S}, \mathcal{A}^N, P, r = (r_1, \cdots, r_N), \gamma\}$, where $N$ is the number of agents. For each $(s, \mathbf{a}) \in \mathcal{S}\times \mathcal{A}^N$, the transition probability from state $s$ to state $s'$ is denoted by $P(s'|s, \mathbf{a})$ when joint action $\mathbf{a}$ is taken, and every agent $i$ receives an individual reward feedback $r_i(s_t, \mathbf{a}_t)$. The action selection rule of agent $i$ can be represented by a mixed/random policy $\pi_i: \mathcal{S} \to \Delta(\mathcal{A})$, where the probability of executing $a_i$ in state $s$ is specified by $\pi_i(a_i|s)$. We denote the joint policy by $\pi = \pi_1 \times \cdots \times \pi_N$.
    
Agent $i$'s individual value function is defined as 
\[
    V_i^{\pi} (s) := \ex{}{\sum_{t=0}^\infty \gamma^t r_i(s_t, \mathbf{a}_t)\ \Big|\ s_0 = s},
\] 
where the joint action $\mathbf{a}_t \sim \pi(\cdot|s_t) = \prod_{i=1}^N \pi_i(a_{t,i}|s_t)$ follows the joint policy $\pi$ and $s_{t+1} \sim P(\cdot|s_t, \mathbf{a}_t)$ is generated by the MDP $\mathcal{M}$ for all $t \ge 0$. $Q$-function is defined in a similar fashion where the initial action is fixed:
\[
    Q_i^{\pi} (s, \mathbf{a}) := \ex{}{\sum_{t=0}^\infty \gamma^t r_i(s_t, \mathbf{a}_t)\ \Big|\ s_0 = s, \mathbf{a}_0 = \mathbf{a}}.
\] 
Every agent $i$ seeks to maximize its individual value function $V_i$ and the game reaches a Nash equilibrium when the policy $\pi$ satisfies
\[
    V_i(\pi_i, \pi_{-i}) \ge V_i(\pi_i', \pi_{-i}),\quad \forall {\pi_i' \in \Delta(\mathcal{A})}
\]
i.e., every agent cannot improve its value function by deviating from the current policy.

\paragraph{Markov Potential Game}
An $N$-agent MDP is a \textit{Markov Potential Game} (MPG) if there exists a potential function $\Phi: \mathcal{S}\times \mathcal{A}^N \to \mathbb{R}$ such that the induced value function $V_\Phi$ satisfies
\[
    V_i^{\pi_{i}, \pi_{-i}}(s) - V_i^{\pi'_{i}, \pi_{-i}}(s) = V_\Phi^{\pi_{i}, \pi_{-i}}(s) - V_\Phi^{\pi'_{i}, \pi_{-i}}(s),
\]
for arbibrary $\pi_i, \pi'_i$ and $\pi_{-i}$. Here, $V_\Phi$ is given by 
\[
    V_\Phi^{\pi} (s) := \ex{}{\sum_{t=0}^\infty \gamma^t \Phi(s_t, \mathbf{a}_t)\ \Big|\ s_0 = s}.
\]
% Nash equilibrium policy is guaranteed to exist in a Markov potential game, e.g., the policy that achieves maximal value in $V_\Phi$ \cite{monderer1996potential}. It is worth noting that there may exist multiple NEs in a potential game.

\subsection{Independent natural policy gradient method}


\subsection{Asymptotic global convergence of INPG}

compare with \citet{fox2021independent}


